Vision-Based Navigation I: A navigation filter for fusing DTM/correspondence updates

An algorithm for pose and motion estimation using corresponding features in images and a digital terrain map is proposed. Using a Digital Terrain (or Digital Elevation) Map (DTM/DEM) as a global reference enables recovering the absolute position and orientation of the camera. In order to do this, the DTM is used to formulate a constraint between corresponding features in two consecutive frames. The utilization of data is shown to improve the robustness and accuracy of the inertial navigation algorithm. Extended Kalman filter was used to combine results of inertial navigation algorithm and proposed vision-based navigation algorithm. The feasibility of this algorithms is established through numerical simulations.

==> ftslru.tex <==
%\maketitle

\pagestyle{empty}
\thispagestyle{empty}
%\documentstyle[12pt,twoside]{article}
%\pagestyle {empty}
%\begin{document}
%\renewcommand{\baselinestretch}{1}
\centerline{\large\bf }
\vspace{0.2cm}
\centerline{\large\bf }
\vspace{2.5cm}
\centerline{\Large\bf  Навигационный фильтр Калмана для }
\centerline{\Large\bf  коррекции ошибок инерциальной навигации}
\centerline{\Large\bf с помощью Цифровой Карты Ландшафта}
\centerline{\Large\bf  и соответствующих точек на кадрах фильма.}
\vspace{2.0cm}
\centerline{Купервассер Олег Юрьевич, Воронов Владимир
Владимирович }
\vspace{0.7cm}
\centerline{\bf }
\vspace{0.4cm}
\centerline{\em группа компаний Транзас}
\centerline{\em Москва, Россия}
\centerline{\em Email: olegkup@yahoo.com}
\par
\vspace{2.0cm}


$$    $$
$$    $$
$$    $$
$$    $$
\centerline{\em Август 2011}
\par
\vspace{0.8cm}
%\renewcommand{\baselinestretch}{1.9}
\newpage
%\end{document}


==> olegKalman_2.tex <==



\begin{abstract}

Предложен алгоритм для нахождения позиции, ориентации и оценки
движения, использующий соответствующие точки в изображениях и
цифровую карту ландшафта. Использование Цифровой Карты Ландшафта
(ЦКЛ) как глобальной справочной информации позволяет
восстановление абсолютной позиции и ориентации камеры. Чтобы
сделать это, ЦКЛ используется, чтобы сформулировать дополнительные
ограничения между соответствующими точками в двух последовательных
кадрах. Использование этих данных позволяет улучшить надежность и
точность инерциального навигационного алгоритма. Расширенный
фильтр  Калмана использовался, чтобы объединить результаты
инерциального навигационного алгоритма и навигационного алгоритма,
 основанного на компьютерном зрении. Выполнимость этого алгоритма продемонстрирована путем численного моделирования.

\end{abstract}



\section{Введение.}
\label{Introduction}

Основанные на системе технического зрения алгоритмы были главной исследовательской проблемой в
течение прошлых десятилетий. Два единых подхода для навигационной проблемы существуют: наземные
ориентиры и интеграция собственного движения. В подходе, основанном на наземных ориентирах,
несколько характерных объектов находятся на плоскости изображения и сверяются по их известному
 трехмерному местоположению.
 Используя 2-ые и трехмерные данные, могут быть получены положение и ориентация камеры.
  Немного примеров для таких алгоритмов - \cite{bib:Liu}, \cite{bib:David}.
  Как только наземные ориентиры были найдены, нахождение положения и ориентации камеры просто и
  может быть достигнуто весьма точно. Основная трудность - обнаружение наземных ориентиров  и
   нахождение их правильного соответствия к объектам из известного набора.

В методе интеграции собственного движения, движение камеры относительно себя самой оценивается.
 Движение эго может быть получено из поля оптического потока, или из приборов, таких как акселерометры и
 гироскопы. Как только собственное движение было получено, можно интегрировать это движение и найти путь камеры.
 Один из коэффициентов, которые делают этот подход привлекательным, - то, что никаких наземных ориентиров не нужно
  находить, в отличие от предыдущего подхода. Несколько алгоритмов оценки собственного движения могут быть найдены
  в \cite {bib:Barron}, \cite {bib:Tian}, \cite {bib:Chiuso}, \cite {bib:Irani}.

   Недостаток метода интеграции собственного движения происходит из того обстоятельства, что маленькие
    ошибки суммируются во время процесса интеграции. Следовательно, ошибка предполагаемого положения и
    ориентации камеры накапливается и происходит уменьшение точности оценки позы с течением времени.
     Если такой подход используется, было бы желательно уменьшить накопление ошибки, активизируя, время
     от времени, дополнительный алгоритм, который оценивает позу непосредственно. В \cite {bib:Sim}
     предлагается такая навигационная система. В этой работе, также как и в настоящей работе, накопление
      ошибки исправляется, используя Цифровую Карту Ландшафта (ЦКЛ). ЦКЛ - дискретное представление топографии
       наблюдаемой местности. Оно содержит высоту над уровнем моря ландшафта для каждого географического
        местоположения. В \cite {bib:Sim} кусок местности был восстановлен, используя 'структуру из движения'
        (СИД) алгоритм, и согласован c ЦКЛ, чтобы получить позу камеры. Использование алгоритма СИД, который не использует информацию, полученную из ЦКЛ, а скорее основывает свою оценку на одном только поле оптического потока, может быть подвержено тому же критическому анализу, что и сам алгоритм СИД \cite {bib:Oliensis}.

Алгоритм, представленный в этой работе, не требует промежуточной явной реконструкции трехмерного мира. Комбинируя информацию из ЦКМ непосредственно с информацией из изображений, алгоритм хорошо обусловлен и генерирует точные оценки для разумных сценариев и разумных ошибок. В данной работе это требование исследуется, выполняя анализ ошибок на алгоритма, выделенном выше. Определяя соответствующие характеристики этих источников ошибок, получаем выражение для неопределенности позы и движения камеры и затем изучаем влияние различных коэффициентов, используя обширное числовое моделирование.




\section{Определение и описание проблемы.}
\label{Problem Definition and Notations}

 Проблема может быть кратко описана следующим образом: В любой момент времени $t$, система координат $C(t)$ установлена на камеру таким способом, что $Z$-ось совпадает с оптической осью, и начало координат совпадает с центром проектирования камеры. В этот момент времени камера расположена в некотором географическом местоположении $p(t)$ и имеет данную ориентацию $R(t)$ относительно глобальной координатной системы $W$ ($p(t)$ - трехмерный вектор, $R(t)$ - ортонормальная матрица вращения). $p(t)$ и $R(t)$ определяют преобразование из координатной системы камеры $C(t)$ в глобальную координатную систему $W$, где, если ${}^{\CCC}v$ и ${}^{\CCC}v$ являются векторами в $C(t)$ и $W$ соответственно, то ${}^{\WWW}v=R(t){}^{\CCC}v+p(t)$.

Рассмотрим теперь два последовательных момента времени $t_1$ и $t_2$: преобразование из $C(t_1)$ в $C(t_2)$ дано вектором сдвига $\Delta p (t_1,t_2)$ и матрицей вращения $\Delta R(t_1, t_2)$ таким образом, что ${}^{\Ctb}v =\Delta R\left({t_1, t_2} \right){}^{\Cta}v +\Delta p\left({t_1, t_2}\right)$. Для грубой оценки позы камеры в $t_1$ и собственное движение камеры между двумя моментами времени - $p_E(t_1)$, $R_E(t_1)$, $\Delta p_E(t_1, t_2)$ и $\Delta R_E(t_1, t_2)$  используются. (Символ "$E$" для нижнего индекса обозначает, что это оценочная (estimated) величина.)

Также используется поле оптического потока: $\left \{{u_i(t_k)}\right\}$ $(\textit{i=1 {\ldots} n, k=1,2})$. Для $i$'th характерная точка местности, $u_i(t_1)\in{\mathbb R}^2$ и $u_i(t_2)\in{\mathbb R}^2$ представляют её местоположение на первом и втором кадре соответственно.

Используя вышеупомянутые обозначения, цель предложенного алгоритма
состоит в том, чтобы оценить истинной позу камеры и её собственное
движение: $p(t_1)$, $R(t_1)$, $\Delta p(t_1, t_2)$ и $\Delta
R(t_1, t_2)$ используя поле оптического потока $\left\{ {u_i (t_k
)} \right\}$, ЦКЛ и приблизительные начальные условия: $p_E(t_1)$,
$R_E(t_1)$, $\Delta p_E(t_1, t_2)$ и $\Delta R_E(t_1, t_2)$.



\section{Навигационный алгоритм.}

Следующий раздел описывает навигационный алгоритм, который оценивает вышеупомянутые параметры. Поза и движение эго камеры получены, используя ЦКЛ и поле оптического потока для двух последовательных кадров. В отличие от метода наземных ориентиров никакие характерные ориентиры не должны быть обнаружены и распознаны. Только соответствие между двумя последовательными изображениями должно быть найдено, чтобы получить поле оптического потока. Как было упомянуто в предыдущем разделе, грубая оценка искомых параметров используется как первое приближение. Однако, так как алгоритм только используют это как начальное приближение и повторно вычисляет позу и движение непосредственно, никакое сложение предыдущих ошибок не будет иметь место, и точность будет сохраняться.

Новый подход основан на следующем наблюдении. Так как ЦКЛ предоставляет информацию о структуре наблюдаемого ландшафта, глубину наблюдаемых характерных точек местности определяет поза камеры. Следовательно, учитывая позу и движение камеры, поле оптического потока может быть однозначно определено. Целью алгоритма является нахождение позы и движения, которые приводят к полю оптического потока наиболее близкому, насколько это возможно, к найденному выше полю оптического потока.

Единичный вектор из поля оптического потока будет использоваться,
чтобы определить ограничения на позу камеры и её движение. Пусть
${}^{\WWW}G\in {\mathbb R}^3$ является местоположением характерной
точки местности в трехмерном пространстве. В два различные момента
времени $t_1 $ и $t_2 $, эта характерная точки местности
проектируется на плоскость изображения камеры в точки $u(t_1)$ и
$u(t_2)$. Используя модель дырочной камеры, получаем
$u(t_1),u(t_2) \in {\mathbb R}^2$. Позвольте ${}^{\CCC}q(t_1)$ and
${}^{\CCC}q(t_2)$ быть гомогенными представлениями этих
местоположений. Также можно описать эти вектора как вектора из
оптического центров камер к точкам проектирования на плоскости
изображений. Используя начальную оценку позы камеры в $t_1$,
линия, проходящая через $p_E (t_1)$ и ${}^{\CCC}q(t_1)$, может
быть пересечена с ЦКЛ. Любой алгоритм трассировки лучей может
использоваться для этой цели. Местоположение этого пересечения
обозначено как ${}^{\WWW}G_E$. Символ "$E$" нижнего индекса
проясняет тот факт, что эта точка местности - предполагаемое
местоположение для характерной точки, который вообще будет
отличаться от истинного местоположения характерной точки
${}^{\WWW}G$. Различие между истинным и оцененным местоположением
происходит из двух основных источников: ошибка в начальном
предположении для позы и ошибка в определении ${}^{\WWW}G_E$,
вызванной дискретизацией ЦКЛ и основными погрешностями. Для
разумных ошибок начального положения и ЦКЛ - связанных ошибок, две
точки ${}^{\WWW}G_E$ и ${}^{\WWW}G$ должны быть достаточно
близким, чтобы позволить линеаризацию ЦКЛ вокруг ${}^{\WWW}G_E$.
Обозначая $N$ нормаль плоскости, касательной к DTM в точке
${}^{\WWW}G_E$, можно написать:

\begin{equation}
\label{eq1} N^T({ }^{\WWW}G-{ }^{\WWW}G_E )\approx 0
\end{equation}

Истинная характерная точка местности ${}^{\WWW}G$ может быть
описана, используя истинные параметры позы:

\begin{equation}
\label{eq2} { }^{\WWW}G=R(t_1 )\cdot { }^{\CCC}q(t_1 )\cdot
\lambda \;+\;p(t_1 )
\end{equation}

Здесь, $\lambda$ обозначает глубину характерной точки (то есть расстояние от точки до плоскости изображения, спроектированное на оптическую ось). Подставляя (\ref {eq2}) в (\ref {eq1}):

\begin{equation}
\label{eq3} N^T(\lambda \cdot R(t_1 )\cdot { }^{\CCC}q(t_1
)\;+\;p(t_1 )\; -\; { }^{\WWW}G_E )=0
\end{equation}

Из этого выражения глубина истинной характерной точки может быть рассчитана, используя оценочное положение характерной точки:

\begin{equation}
\label{eq4} \lambda =\frac{N^T{ }^{\WWW}G_E -N^Tp(t_1 )}{N^TR(t_1
){ }^{\CCC}q(t_1 )}
\end{equation}

Подстановкой (\ref{eq4}) обратно в (\ref{eq2}) получаем:

\begin{equation}
\label{eq5} { }^{\WWW}G=R(t_1 ){ }^{\CCC}q(t_1 )\cdot \left(
{\frac{N^T{ }^{\WWW}G_E -N^Tp(t_1 )}{N^TR(t_1 ){ }^{\CCC}q(t_1 )}}
\right)+p(t_1 )
\end{equation}

Чтобы упростить обозначения, $R(t_i)$ будет заменен $R_i$ и аналогично для $p(t_i) $ и $q(t_i)$ $i=1,2$. $\Delta R(t_1, t_2)$ и $\Delta p(t_1, t_2)$ будут заменены на $R_{12}$ и $p_ {12}$ соответственно. Верхний индекс, описывающий систему координат, в которой дан вектор, будет также опущен, за исключением случаев, где требуется особое внимание к описываемым системам координат. Обычно, $p_{12} $ и $q$'s находится в системе координат камеры, в то время как остальная часть векторов дана в глобальной системе координат. Используя упрощенные обозначения, (\ref {eq5}) может быть переписано как:

\begin{equation}
\label{eq6} G\;=\;\frac{R_1 q_1 N^T}{N^TR_1 q_1 }G_E
\;-\;\frac{R_1 q_1 N^T}{N^TR_1 q_1 }p_1 \;+\;p_1
\end{equation}

Для того, чтобы получить более простое выражение определим следующий проектирующий оператор:

\begin{equation}
\label{eq7} \mathcal P(u,s)\buildrel\textstyle.\over= \left( {{\rm
I}-\frac{us^T}{s^Tu}} \right)
\end{equation}

Этот оператор проектирует вектор на нормаль подпространства к $s$, вдоль направления $u$. Как иллюстрация, это просто проверить, что $s^T\cdot\mathcal P(u, s)v\equiv 0$ и $\mathcal P(u, s)u\equiv 0$. Добавляя и вычитая $G_E$ к (\ref {eq6}), после переупорядочения:

\begin{equation}
\label{eq8} G=G_E +\left[ {{\rm I}-\frac{R_1 q_1 N^T}{N^TR_1 q_1
}} \right]p_1 -\left[ {{\rm I}-\frac{R_1 q_1 N^T}{N^TR_1 q_1 }}
\right]G_E
\end{equation}

Используя проектирующий оператор, (\ref{eq8}) становится:

\begin{equation}
\label{eq9} G=G_E +\mathcal P(R_1 q_1 ,N)\left( {p_1 -G_E }
\right)
\end{equation}

У вышеописанного выражения есть ясная геометрическая интерпретация
(см. Рис.\ref{geometricalFig}). Вектор из $G_E$ к $p_1$
проектируется на касательную плоскость. Проектирование идет вдоль
направления $R_1 q_1$, которое является направлением луча из
оптического центра камеры ($p_1$), проходящего через
соответствующую точку изображения.

\begin{figure}[tbp]
\centering
\includegraphics[width=80mm,height=50mm]{figures/geometrical.eps}
\caption{Геометрическое описание выражения (\ref{eq9}) используя
проектирующий оператор (\ref{eq7})} \label{geometricalFig}
\end{figure}


Наш следующий шаг будет перенос $G$ из глобальной системы координат - $W$ в систему координат  первой камеры $C_1$ и затем к системе координат  второй камеры $C_2$. Так как $p_1$ and $R_1$ описывают преобразование из $C_1$ в $W$, мы будем использовать обратное преобразование:

\begin{equation}
\label{eq10} { }^{\Cb}G=p_{12} +R_{12} \left( {R_1^T \left( {G-p_1
} \right)} \right)
\end{equation}

Подстановка (\ref{eq9}) в (\ref{eq10}) дает:

\begin{equation}
\label{eq11} { }^{\Cb}G=p_{12} +R_{12} \mathcal L\left( {G_E -p_1
} \right)
\end{equation}

$\mathcal L$ в написанном выше выражении представляет:

\begin{equation}
\label{eq12} \mathcal L=\frac{q_1 N^T}{N^TR_1 q_1 }
\end{equation}

Можно интерпритировать $\mathcal L$ как оператор  обратный  к $\mathcal P$: он проектирует векторы на луч, продолжающий $R_1 q_1$ вдоль плоскости, ортогональной к $N$.

$q_2$ - проекция истинной характерной точки местности $G$. Таким образом, векторы $q_2$ и ${}^{\Cb}G$ должны совпасть. Это наблюдение может быть выражено математически, проектируя ${}^{\Cb}G$ на продолжение луча $q_2$:

\begin{equation}
\label{eq13} { }^{\Cb}G=\frac{q_2 }{\left| {q_2 } \right|}\cdot
\left( {\frac{q_2 ^T}{\left| {q_2 } \right|}\cdot { }^{\Cb}G}
\right)
\end{equation}

В выражении (\ref{eq13}), ${q_2 ^T} \mathord{\left/ {\vphantom {{q_2 ^T} {\left| {q_2 } \right|}}} \right. \kern-\nulldelimiterspace} {\left| {q_2} \right|}\cdot {}^{\Cb}G$ является величиной ${ }^{\Cb}G$'s прекции на $q_2$. Преобразуя (\ref{eq13}) и используя проектирующий оператор, мы получаем:

\begin{equation}
\label{eq14} \left[ {{\rm I}-\frac{q_2 \cdot q_2 ^T}{q_2 ^T\cdot
q_2 }} \right]\cdot { }^{\Cb}G\quad =\quad \mathcal P(q_2 ,q_2
)\cdot { }^{\Cb}G\quad =\quad 0
\end{equation}

${ }^{\Cb}G$ является проекцией на ортогональную компонент $q_2$. Так как ${ }^{\Cb}G$ и $q_2 $ должны совпадать,это проектирование должно давать нулевой вектор. Подстановка (\ref{eq11}) в (\ref{eq14}) приводит к нашему окончательному ограничению:

\begin{equation}
\label{eq15} \mathcal P(q_2 ,q_2 )\left[ {p_{12} +R_{12} \mathcal
L\left( {G_E -p_1 } \right)} \right]=0
\end{equation}

Это ограничение включает позицию, ориентацию и собствнное движение, определяемое на основе двух кадров камеры. Хотя оно включают трехмерные вектора, ясно, что его ранг не может превысить двойку из-за использования $\mathcal P$, который проектирует ${\mathbb R}^3$ на двумерное подпространство.

Такое ограничение может быть установлено для каждого вектора в поле оптического потока, пока не будет получена несингулярная система. Так как двенадцать параметров должны быть оценены (шесть для позы и шесть для собственного движения), по крайней мере, шесть векторов оптического потока требуются для решения системы. Но это - правильное заключение для нелинейной проблемы. Если мы используем метод итераций Гаусса-Ньютона, то делаем линеаризацию нашей проблемы около приближенного решения. Найденная матрица будет всегда сингулярной для шести точек (с нулевым детерминантом), как численное моделирование демонстрирует. Таким образом, необходимо использовать, по крайней мере, семь точек, чтобы получить несингулярное линейное приближение. Обычно, чем больше векторов будет использоваться, чтобы определить переопределенную систему, тем более устойчиво решение. Внимание должно быть привлечено к факту, что было получено нелинейное ограничение. Таким образом, итерационная схема будет использоваться, чтобы решить эту систему. Устойчивый алгоритм, который использует итерации Гаусса-Ньютона и М-оценщик описан в \cite{bib:technicalReport}. Мы начинаем использовать метод Levenberg-Marquardt, если метод Гаусса-Ньютона после нескольких итераций прекратил сходиться. Эти два алгоритма реализованы в функции lsqnonlin() пакета Matlab. Применимость, точность и надежность алгоритма были проверены через численное моделирование и лабораторные эксперименты.

Более удобно использовать более устойчивое для итераций решение, эквивалентное уравнению (\ref{eq15}):

\begin{equation}
\label{eq166} \quad \mathcal P(q_2 ,q_2 )\left[ {p_{12} +R_{12}
\mathcal L_i \left( {G_{E_i } -p_1 } \right)} \right]/|{
}^{\Cb}G|=0
\end{equation}

Использование этой нормализованной формы уравнений предотвращает получение неверного тривиального решения, когда две позиции находятся в единой точке на местности.

\section{ Навигационный алгоритм, основанный на компьютерном зрении, для коррекции инерциальной навигации с помощью фильтра Калмана.}
\label{sec_Vision-based}

Основанные на компьютерном зрении навигационные алгоритмы были
главной исследовательской проблемой в течение прошлых десятилетий.
Алгоритм, используемый в этой статье, основан на  геометрии многих
изображений и карте местности. С помощью этого метода мы получаем
позицию и ориентацию наблюдающей камеры. С другой стороны мы
получаем те же самые данные из инерциальных навигационных методов.
Чтобы скорректировать эти два результата, используется фильтр
Калмана. Мы используем в этой статье расширенный фильтр Калмана
для нелинейных уравнений \cite{bib:my1}.

Для инерциальных навигационных вычислений использовался
Инерциальный Навигационный Системный Пакет для Matlab
\cite{bib:my2}.

Вход фильтра Калмана состоит из двух частей. Первый - переменные
$X$ для уравнений движения. В нашем случае это - инерциальные
навигационные уравнения. Вектор $X$ состоит из пятнадцати
компонентов: $ [\delta x\: \delta y\: \delta z\: \delta V_x
\:\delta V_y \: \delta V_z \:\delta\phi \:\delta\theta
\:\delta\psi\: a_x \:a_y \:a_z \:b_x \:b_y \:b_z] $. Координаты
$\delta x\: \delta y\: \delta z$ определены как разница между
реальной позицией камеры и позицией, полученный из инерциального
навигационного вычисления. Переменные $\delta V_x \:\delta V_y \:
\delta V_z$ определены как разница между реальной скоростью камеры
и скоростью, полученной из инерциального навигационного
вычисления. Переменная $\delta\phi \:\delta\theta \:\delta\psi$
определена как углы Эйлера матрицы $D_r*D_c^T$. Здесь $D_r$
матрица определена реальными углами Эйлера камеры относительно
локальной системы координат (L-frame). С другой стороны $D_c$
матрица определена углами Эйлера камеры относительно локальной
системы координат (L-frame), полученными из инерциального
навигационного вычисления. Необходимо обратить внимание, что
найденные углы Эйлера $\delta\phi \: \delta\theta \: \delta\psi$
НЕ эквивалентны разнице между реальными углами Эйлера и углами
Эйлера, полученными из инерциального навигационного вычисления.
Однако для маленьких значений $\delta\phi \: \delta\theta \:
\delta\psi$ попрвки к этим углам могут быть добавлены линейно и
таким образом эти углы могут использоваться в фильтре Калмана в
случае маленьких ошибок. Такой выбор углов сделан, поскольку
формулы, описывающие их эволюцию, намного более просты, чем
формулы, описывающие эволюцию разницы между углами Эйлера.
Переменные $a_x \:a_y \:a_z$ определены вектором смещения
ускорения в инерциальных навигационных измерениях. Переменные
$\:b_x \:b_y \:b_z$ определены вектором гироскопического смещения
в инерциальных навигационных измерениях.

Второй вход фильтра Калмана - $Z$-результат измерений, основанных на навигационных алгоритмах компьютерного зрения. Вектор $Z$ состоит из шести компонентов $[\delta x_m\: \delta y_m\: \delta z_m\: \delta\phi_m \:\delta\theta_m\:\delta\psi_m]$. Координаты $\delta x_m\: \delta y_m\: \delta z_m$ являются разницей между позицией камеры, измеренной  на основе навигационного алгоритма компьютерного зрения, и позицией, полученный из инерциального навигационного вычисления. Переменная $\delta\theta_m\:\delta\psi_m$ определена как углы Эйлера матрицы $D_m*D_c^T$. Здесь $D_m$ матрица определена углами Эйлера камеры относительно относительно локальной системы координат (L-frame), измеренных  на основе навигационного алгоритма компьютерного зрения. С другой стороны $D_c$ матрица определена углами Эйлера камеры относительно локальной системы координат (L-frame),  полученными из инерциального навигационное вычисления. Пусть переменная $k$ определяет число шагов для дискретизации времени, используемых в фильтре Калмана.

Мы полагаем, что ошибки между значениями, плученными из инерциального навигационного вычисления, и реальными значениями линейно зависят от шума. Соответствующая ковариационная матрица шума обозначена $Q_k$. Диагональные элементы $Q_k$ соответствуют скорости, определяются шумом ускорения и пропорциональны $dt^2$: $Q_V \sim dt^2$, где $dt$ интервал времени между $t_k$ и $t_{k-1}$: $dt=t_k-t_{k-1}$. Диагональные элементы $Q_k$ соответствуют углам Эйлера, определяются гироскопическим шумом и пропорциональны $dt$: $Q_A \sim dt$.

Мы предполагаем, что также ошибки между значениями, полученными на основе навигационного алгоритма компьютерного зрения, и реальными значениями линейно зависят от шума. Соответствующая ковариационная матрица шума обозначена $R_k$. Анализ ошибок, дающий эту матрицу, описан в \cite{bib:my3}.

Уравнения фильтра Калмана описывают как эволюцию $апостериорных$  оценок состояния $X_k$, описанных выше,так и эволюцию $апостериорной$  ковариационной матрицы $P_k$ для переменных $X_k$.

Чтобы написать уравнения фильтра Калмана, мы должны определить еще две 15x15 матрицы: $H_k$ и $A_k$. Матрица $H_k$ является якобианом измерения, описывающая связь между предсказанным измерением $H_k*X_k$ и фактическим измерением $Z_k$, определенным выше. Диагональные элементы $H_k(1,1)$, $H_k(2,2)$, $H_k(3,3)$, описывающие координату и элементы $H_k(4,7)$, $H_k(5,8)$, $H_k(6,9)$, описывающие углы, равны единице. Остальная часть элементов равна нулю.

$A_k$  матрица Якоби, описывающая эволюцию вектора $X_k$. Точное выражение для этой матрицы является очень сложным, поэтому мы используем приближенную формулу для $A_k$, пренебрегая эффектами кориолиса, вращением Земли и так далее. Позвольте $\phi \: \theta \: \psi$ быть углами Эйлера в L-frame, $dV$ является вектором deltaV, полученным из инерциальных навигационных измерений, $f_{vec}$ вектор ускорения в L-frame, $DCM_{\mbox{b-to-l}}$ - матрица направляющих косинусов (для перевода из координатной системы летательного аппарата в L-frame).

 Формулы определяющие $A_k$, следующие:




\begin{equation}
{\Psi}_{DCM} =\left(
\begin{array}{ccc}

 \cos(\psi)   &     \sin(\psi)   &    0\\
 -\sin(\psi) &     \cos(\psi)   &    0\\
 0           &           0           &    1
\end{array}
\right)\label{eq111.1}
\end{equation}




\begin{equation}
{\Theta}_{DCM} =\left(
\begin{array}{ccc}
 \cos(\theta)   &     0   &    -\sin(\theta)\\
 0 &     1   &    0\\
\sin(\theta)   &   0   & \cos(\theta)
\end{array}
\right)\label{eq112.1}
\end{equation}

\begin{equation}
{\Phi}_{DCM} =\left(
\begin{array}{ccc}

1   &     0   &    0\\
 0        & \cos(\phi)   & \sin(\phi)\\
0        & -\sin(\phi)   & \cos(\phi)
\end{array}
\right)\label{eq113.1}
\end{equation}









\begin{equation}
\label{eq115.1} DCM_{\mbox{b-to-l}}=\Phi_{DCM}\Theta_{DCM}
\Psi_{DCM}
\end{equation}










\begin{equation}
\label{eq116.1}
 f_{vec} = DCM_{\mbox{b-to-l}} \frac{dV}{dt}
\end{equation}









\begin{equation}
{Phi(1:3,4:6) } =\left(
\begin{array}{ccc}
   1   & 0& 0 \\
    0 &     1   & 0\\
    0& 0 &     1
\end{array}
\right)\label{eq117.1}
\end{equation}




\begin{equation}
{Phi(4:6,7:9)} =\left(
\begin{array}{ccc}
   0   & -f_{vec}(3)& f_{vec}(2) \\
    f_{vec}(3) &     0   & -f_{vec}(1)\\
    -f_{vec}(2)& f_{vec}(1) &     0
\end{array}
\right)\label{eq118.1}
\end{equation}


\begin{equation}
Phi(7:9,10:12) = -DCM_{\mbox{b-to-l}} \label{eq119.1}
\end{equation}

\begin{equation}
Phi(4:6,13:15) = -DCM_{\mbox{b-to-l}}\label{eq120.1}
\end{equation}


Остальные элементы матрицы Phi равны нулю.

\begin{equation}
A_k = I + Phi \: dt\label{eq121.1}
\end{equation}























Уравнения фильтра Калмана для временной эволюции следующие

\begin{equation}
X_k^{-}=[0 \: 0\: 0 \: 0\: 0\: 0\: 0\: 0\: 0\: {a_x}_{k-1}\:
{a_y}_{k-1}\: {a_z}_{k-1}\: {b_x}_{k-1} \: {b_y}_{k-1}\:
{b_z}_{k-1}]\label{eq122.1}
\end{equation}

\begin{equation}
P_k^{-}=A_k P_{k-1} A_k^{T}+Q_{k-1}\label{eq123.1}
\end{equation}


Уравнения фильтра Калмана проектируют состояние и ковариационную матрицу с предыдущего временного шага $k-1$  на текущий временной шаг $k$.


Уравнения фильтра Калмана для измерения следующие:



\begin{equation}
K_k=P_k^{-} H_k^T (H_k P_k^{-} H_k^T +R_k)^{-1}\label{eq124.1}
\end{equation}

\begin{equation}
X_k=X_k^{-} + K_k (Z_k-H_k X_k^{-})\label{eq125.1}
\end{equation}



\begin{equation}
P_k=(I - K_k  H_k) P_k^{-} (I - K_k H_k)^T + K_k R_k
K_k^T\label{eq126.1}
\end{equation}



Уравнения  фильтра Калмана для измерения исправляют состояние и ковариационной матрицу в соответствии с измерением $Z_k$.

Найденный вектор $X_k$ используется, чтобы обновить координаты, скорости, углы Эйлера, смещение ускореня и гироскопическое
смещение для инерциальных навигационных вычислений на следующем шаге.

Численные расчеты были реализованны, чтобы исследовать
эффективность фильтра Калмана и чтобы объединить эти два
навигационных алгоритма. На  Рис. \ref{fig:fige1} мы можем видеть,
что для
 откорректированного пути ошибка координаты, полученныя на основе двух навигационных методов с фильтрацией Калмана,
 намного меньше чем инерциальная навигационная ошибка координаты, полученная без фильтра Кальмана.
 Улучшенные результаты с помощью фильтра Калмана были получены также для скорости, несмотря на то,
 что эта скорость не  измеряется напрямую навигационным алгоритмом, использующим компьютерное зрение Рис. \ref{fig:fige2}.

\begin{figure}[htb]
%\centerline{
\centering
%\includegraphics[width=80mm,height=50mm]{figures/geometrical.eps}
\begin{tabular}{c}
 %\psfig{figure=figures/picturex.eps,width=2 in}\\
 \includegraphics[width=80mm,height=50mm]{figures/picturex.eps}\\
 (a) \\
 \includegraphics[width=80mm,height=50mm]{figures/picturey.eps}\\
 %\psfig{figure=figures/picturey.eps,width=2 in}\\
 (b)\\
 %\psfig{figure=figures/picturez.eps,width=2 in} \\
 \includegraphics[width=80mm,height=50mm]{figures/picturez.eps}\\
(c)
\end{tabular}
%}
 \caption
{ Ошибки позиции ((a) для координаты x (b) для координаты y (c)
для координаты z). Ошибки инерциального дрейфа отмечены красной
линией, и ошибки, исправленные видео-навигацией, отмечены синей
линией.} \label{fig:fige1}
\end{figure}


\begin{figure}[htb]
%\centerline{
\begin{tabular}{c}
 \psfig{figure=figures/picturevelINS.eps,width=3 in}\\
 (a) \\
\psfig{figure=figures/picturevelKal.eps,width=3 in}  \\
(b)
\end{tabular}
%}
 \caption
{(a) ошибки скорости для инерциального дрейфа (x y z компоненты), и (b) ошибки скорости, исправленные видео-навигацией (x y z компоненты). }
\label{fig:fige2}
\end{figure}






\section{Выводы}
\label{sec_conclusions}

Алгоритм для оценки позы и движения, использующий соответствующие точки в изображениях и ЦКЛ был представлен с использованием фильтра Калмана. ЦКЛ служит как глобальная справочная информация, и ее данные используются для того, чтобы восстановить абсолютную позицию и ориентацию камеры. В численных расчетах оценка для позиции  и скорости находятся достаточно точно, чтобы предотвратить накопленные ошибки и предотвратить дрейф траектории.

\subsection*{Благодарность}

Мы бы хотели поблагодарить Ронена Лернера, Эхуда Ривлина и Хектора
Ротштейна за очень полезные консультации



\begin{thebibliography}{14}
\small  % Use 9 point text.

%\bibitem{bib:Hartley}
%R.Hartley, A.Zisserman, ``Multiple View Geometry in Computer Vision'', Cambridge university press,
%2000

\bibitem{bib:Oliensis}
John Oliensis, “A critique of structure-from-motion algorithms”,
Computer Vision and Image Understanding, vol. 80, pp. 172–214,
2000

%\bibitem{bib:Haralick}
%R. M. Haralick, C-N. Lee, K. Ottenberg, M. Nolle, ``Review and analysis of solutions of the three
%point perspective pose estimation problem'', International Journal of Computer Vision, vol. 13,
%no. 3, pp. 331-356, 1994

%\bibitem{bib:Alter} T.D. Alter, ``3-D pose from 3 points using
%weak-perspective'', IEEE Transactions on pattern analysis and machine intelligence, vol. 16, no.
%8, 1994

\bibitem{bib:Liu} Y. Liu, M.A. Rodrigues, ``Statistical image analysis for
pose estimation without point correspondences'', Pattern
Recognition Letters, vol. 22, pp. 1191-1206, 2001

\bibitem{bib:David} P. David, D. DeMenthon, R. Duraiswami, H. Samet,
``SoftPOSIT: Simultaneous pose and correspondence determination'',
ECCV 2002, LNCS 2352, pp. 698-714, 2002

%\bibitem{bib:Huang} T. S. Huang, A. N. Netravali, ``Motion and
%structure from feature correspondences: a review'', Proc. Of the IEEE, vol. 82, no. 2, 1994

\bibitem{bib:Barron} J. L. Barron and R. Eagleson, ``Recursive estimation of
time-varying motion and structure Parameters'', Pattern
Recognition vol. 29, no. 5, pp. 797--818, 1996

\bibitem{bib:Tian} T.Y. Tian, C. Tomashi, D.J. Hegger, ``Comparison of
approaches to egomotion computation'', Department of Psychology
and Computer science, Stanford university, CA 94305, 1996

\bibitem{bib:Chiuso} A.Chiuso, S.Soatto, ``MFm: 3-D Motion From 2-D Motion,
Causally integrated over time'', Washington University Technical
Report, 1999

\bibitem{bib:Irani} M. Irani, B. Rousso, S. Peleg, ``Robust Recovery of
Ego-Motion'', Proc. Of CAIP 93, pp. 371-378, 1993

\bibitem{bib:Sim} D.G. Sim, R.H. Park, R.C. Kim, S.U. Lee, I.C. Kim,
``Integrated position estimation using aerial image sequences'',
IEEE transactions on pattern analysis and machine intelligence,
vol. 24, no.1, 2002


\bibitem{bib:technicalReport}
Technical report (to be added after the double-blind review).

\bibitem{bib:HaralickErrorAnalysis}
R. M. Haralick, ``Propagating Covariance In Computer Vision'',
Advances in Image Understanding, Azriel Rosenfeld, Bowyer and
Ahuja, (eds.), IEEE Computer Society Press, pp. 142-157,
Washington, 1996

\bibitem{bib:Rees}
Rees W.G., ``The accuracy of Digital Elevation Models interpolated
to higher resolutions'', International Journal of Remote Sensing
vol. 21 no.1, pp. 7-20, 2000

\bibitem{bib:my1}
Greg Welch and Gary Bishop "An Introduction to the Kalman Filter"
UNC-Chapel Hill TR 95-041,NC 27599-3175 April 5, 2004

\bibitem{bib:my2}
www.GPSSoftNav.com

\bibitem{bib:my3}
Oleg Kupervasser, Ronen Lerner, Ehud Rivlin and Hector Rotstein
"Error Analysis for a Navigation Algorithm based on Optical-Flow
and a Digital Terrain Map" In the Proceedings of the 2008 IEEE/ION
Position, Location and Navigation Symposium, P.1203-1212

\end{thebibliography}

